Study of ttbb and ttW background modelling for ttH analyses

This note presents Monte Carlo generator comparisons of the ttbb and ttW processes at particle level. The aim is to compare the modelling of important backgrounds to ttH measurements in multi-lepton final states and in the ttH(H->bb) decay channel and the treatment of the associated theory uncertainties for a combination of the full Run-2 ttH results from ATLAS and CMS. As a first step, modelling and theory uncertainties as used in ATLAS an CMS are compared in the relevant analysis regions. Significant differences in the treatment of systematic uncertainties between the experiments have been observed in ttbb and ttW. As a first step, ATLAS and CMS agreed on a common reference value of the inclusive ttW cross section to allow direct comparisons between experiments.

==> Makefile <==
BASEDN=LHCHWG_Public_Note_ttbbttW
RUNTEX=pdflatex
RUNBIB=bibtex

all: buildpdf

buildpdf:	*.tex Tex/*.tex bib/*.bib
	$(RUNTEX) $(BASEDN).tex
	$(RUNBIB) $(BASEDN).aux
	$(RUNTEX) $(BASEDN).tex
	$(RUNTEX) $(BASEDN).tex
	echo "\nUndefined references:"
	grep undefined $(BASEDN).log	
	make clean

clean:
	-rm *.aux *.bbl *.blg *.log *.out *.toc


==> Tex/Introduction_approved_ATLAS.tex <==
%-------------------------------------------------------------------------------

\section{Introduction}
\label{sec:intro}


%-------------------------------------------------------------------------------

The search for Higgs boson production in association with a top quark pair (\ttH) in the $H\rightarrow b\bar{b}$~\cite{ttHbb, ttHbbRun2,CMS-PAS-HIG-18-030,CMS-HIG-17-026} and in  multi-lepton final states~\cite{ATLAS-CONF-2019-045,CMS-HIG-19-008} analyses is limited by the modelling uncertainties of the main backgrounds, \ttbb and \ttW, respectively. %, where V denotes either a W or Z boson. 
Examples of tree-level diagrams of these processes are shown in Figure~\ref{intro:sig}. A comparison of available Monte Carlo (MC) generators is thus performed to study modelling differences. Comparisons of observables are made at particle level, in a phase space similar to the reference measurements. %Differences in the object and event selection were made to the recently published $\text{H}\rightarrow b\bar{b}$ and $\text{H}\rightarrow$ multi-lepton analyses. 
The goal is to provide input to a discussion on a common strategy for ATLAS and CMS modelling uncertainties in the $\ttH(b\bar{b})$ and $\ttH$(multi-lepton) analyses. Comparisons of \ttbb distributions will be presented in Section~\ref{sec:ttbb} and of \ttW distributions in Section~\ref{sec:ttW}.%, comparison and discussion of different ways of systematics treatment in Section~\ref{sec:syst}.

\begin{figure}[!htb]
  \centering
  \begin{tabular}{ccc}
    \includegraphics[width=0.35\textwidth]{Plots/ttbb/ttbb}
    &&
    \includegraphics[width=0.35\textwidth]{Plots/ttW/ttW.png} \\
  \end{tabular}
  \caption{Examples of tree-level Feynman diagrams for \ttbb (left) and \ttW (right). \label{intro:sig}}
\end{figure}

==> Tex/systematics.tex <==
\subsection{Comparison of systematics contributions}
\label{sec:syst}


In the study presented here, the uncertainty due to missing  higher order corrections is estimated by varying renormalisation and factorisation scales simultanously by a factor of 0.5 and 2.0 with respect to the central value. In Figure~\ref{syst:4j12b} 
 %These uncertainties are estimated varying the renormalisation and factorisation scale independently by a factor of 0.5 and 2.0 with respect to the central value. 
%The generated samples come with 7-point scale variations of the renormalisation ($\mu_{R}$) and the factorisation scale ($\mu_{F}$), i.e. pairwise variations of
 the distributions for all combinations of variations of the renormalisation and factorisation scales are shown which motivates this choice. For the observables studied, the largest variation is obtained in almost all bins when varying both scales simultaneously in the same direction ([$\mu_{R}$,$\mu_{F}$] =[0.5,0.5] and [2,2]). Therefore these variations is taken as a  single nuisance parameter in the  profile likelihood fit to data in the  data analysis. Also note that  the variation of \muR dominates the difference to the central value.


%There are different ways of implementation of these uncertainties into the statistical model: separate nuisance parameter for each of six variations, taking the envelope of largest uncertainties (per-bin) - single nuisance parameter, and grouping up and down variation for one scale (for example $\mu_{R}^{up}$=[0.5,1] and $\mu_{R}^{down}$=[2,1]) - three nuisance parameters.

%\subsection{Proposal}
%The scope of this note to discuss available options and to suggest common treatment of the uncertainties.
%As shown on Figure~\ref{syst:4j12b}, combination of simultaneous variation of the renormalisation and factorisation scales ($\mu_{RF}^{up}$=[0.5,0.5] and $\mu_{RF}^{down}$[2,2]) has largest contribution for most of the distributions. 
%muR Up/Down and muRF Up/Down will be basically degenerate (for instance) ?.. so this will be 
%Trying to combine a double counting.
%Comparing the single ($\mu_R$ and $\mu_F$) variations we see that the $\mu_R$ are dominant then the combined variation ($\mu_{RF}$) will also be dominated by $\mu_R$ and therefore lead to a large double counting. 
%Therefore, we have two options:
%\begin{itemize} 
%\item use $\mu_{RF}$ as a single nuisance parameter - easiest implementation, avoids double counting
%\item omit $\mu_{RF}$ and use combination of single variations $\mu_R$ and $\mu_R$ i.e. 2 NPs total - compromise between sufficient flexibility in the fit and no over-inflating the uncertainties.
%\end{itemize} 

\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttw/syst/c_Region_0_nJets}
\includegraphics[width=0.45\textwidth]{Plots/ttw/syst/c_Region_1_nJets}\\
\includegraphics[width=0.45\textwidth]{Plots/ttw/syst/c_Region_0_HT_jets}
\includegraphics[width=0.45\textwidth]{Plots/ttw/syst/c_Region_1_HT_jets}\\
  \caption{Scale uncertainty systematic variation comparison. Distribution of the jet multiplicities (top) and the scalar sum of jets transverse momentum, $HT^{\text{jets}}$ (bottom), for the Region 1 with $N_{b-\mathrm{jets}}=$1 (left) and Region 2 with  $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets. All distributions are normalised to YR4 cross section of 600.8 fb. The ATLAS sample is used to demonstrate the issue.  \label{syst:4j12b}}
\end{figure}

==> Tex/ttW_approved_ATLAS.tex <==
\section{Comparison of MC predictions for the $t\bar{t}W$ process}
\label{sec:ttW}

%The CMS \cite{CMS-HIG-19-008} and ATLAS measusurements \cite{ATLAS-CONF-2019-045} of  the ttH production cross section in the Higgs decay channel to several leptons show that the dominant background stems from ttW production. In order to describe this background different MC models are used for the ongoing and published measurements by the two experiments and be described in the following.

% Josh adding reference to new CMS ttW measuremnt:
The CMS \cite{CMS-HIG-19-008} and ATLAS experiments  \cite{ATLAS-CONF-2019-045} measured the \ttH production cross section in multi-lepton final states
 which are primarily sensitive to the decays of H$\rightarrow WW^*$, H$\rightarrow \tau \tau$ and H$\rightarrow ZZ^*$. The dominant background in these measurements stems from \ttW production. These measurements along with the recent CMS measurement of \ttW production~\cite{CMS-PAS-TOP-21-011} show some tension with the SM predictions. In order to describe this background, different MC models are used for the future and published measurements by the two experiments and will be described in the following.


\subsection{MC generator set-ups}
%\subsubsection*{ATLAS setup}
%ATLAS uses two MC generators.  % are compared in this study.
%ATLAS has studied three MC generator setups.  % are compared in this study.

%The nominal sample for inclusive \ttW production was generated using the \textsc{Sherpa}~2.2.8~\cite{Gleisberg:2008ta} generator with the NNPDF3.0 NLO PDF set.
The nominal sample for inclusive \ttW production was generated using the \textsc{Sherpa}~2.2.10~\cite{Sherpa,Gleisberg:2008ta} generator with the NNPDF3.0 NLO PDF set.
The matrix element (ME) was calculated for up to one additional parton at NLO and up to two partons at LO using
\textsc{Comix}~\cite{Gleisberg:2008fv} and \textsc{OpenLoops}~\cite{Cascioli:2011va}, and merged with the \textsc{Sherpa} parton shower~\cite{Schumann:2007mg} using the \textsc{MEPs@Nlo} prescription~\cite{Hoeche:2012yf} with a merging scale of 30 GeV.
The choice of renormalization and factorization scales is $\muR = \muF = H_\textrm{T}$/2, where $\HT$ is defined as the scalar sum of the transverse masses $\sqrt{\pt^2+m^2}$ of all final state particles.
Detailed information of the \textsc{Sherpa} sample is  listed in Table~\ref{tab:mcconfig}.
Systematic uncertainties due to missing higher-order QCD corrections are estimated in the nominal sample by varying the factorization and renormalization scales together with  \alphas in the parton shower  by a factor of 0.5 (2.0) with respect to the central value.
% called further SherpaScaleDown (SherpaScaleUp). % ($\mu_R=\mu_F=0.5$ and $\mu_R=\mu_F=2.0$ ).

In addition to this nominal prediction at NLO in the strong coupling a separate sample is produced which contains also higher order corrections relating to electroweak (EW) contributions. These are added in two ways. First, through event-by-event correction factors 
%derived using the virtual additive corrections in the formalism described in Ref.~\cite{Kallweit:2015dum}. These event weights provide 
of the order $\alpha^3$ and $\alpha^{2}\alphas^{2}$  where $\alpha$ ($\alphas$) refers to the EW (QCD) coupling constant.  Secondly, sub-leading EW corrections at order $\alpha^{3}\alphas$ ~\cite{Frederix:2017wme}
are introduced via the addition of an independent \textsc{Sherpa}~2.2.10 sample  produced at LO in QCD for this final state. This sample is marked as "QCD+EW" in the following. 
 

 %contribute larger corrections to the typical leading corrections~\cite{Frederix:2017wme}, these corrections are introduced via the addition of an independent \textsc{Sherpa}~2.2.10 prediction produced at LO in QCD for this final state and marked as "QCD+tree-level EW" in the following. 


Uncertainties associated with the modelling of additional QCD radiation have been estimated by comparing the nominal \ttW prediction with that of an alternative sample that was generated at NLO with the \textsc{MadGraph5\_aMC@NLO}~2.3.3~\cite{Alwall_2014} generator using the same scale choice as for the nominal   sample and PDF set NNPDF3.0NLO, and interfaced to \textsc{Pythia}~8.210~\cite{Sjostrand:2014zea} in combination with the A14 tune~\cite{ATL-PHYS-PUB-2014-021}.

A \ttW prediction was produced using the \textsc{MadGraph5\_aMC@NLO}~2.9.3 program to generate \ttW production with up to one additional parton  in the final state at NLO accuracy in the strong coupling. The renormalization and factorization scales are the same as in the nominal sample. The showering and subsequent hadronization is performed using \textsc{Pythia}~8.245\cite{Sjostrand:2014zea} with the A14 tune~\cite{ATL-PHYS-PUB-2014-021}.
%and the NNPDF2.3lo PDF set~\cite{Ball:2012cx} with $\alpha_S = 0.130$. 
The different jet multiplicities are merged using the FxFx NLO matrix-element and parton-shower merging prescription~\cite{Frederix:2012ps}, see detailed description in \cite{atlasFXFXPub}. 

The configurations of the samples are summarised in Table~\ref{tab:mcconfig}.


\newpage
%\begin{table}[hb]
%\begin{center}
%\caption{\label{tab:sherpadetails}Details of ATLAS Sherpa event generation of the \ttW processes.}
%\vspace{0.25cm}
%{\small
%\setlength\tabcolsep{1.5pt}
%\begin{tabular}{l|l}
%\hline\hline
%Generator & ME scale & Parton shower & PDF & Tune  \\
%& (alternative) & (alternative) & & \\
%Merging & \textsc{MEPs@Nlo} prescription with a merging scale of 30 GeV \\
%Scale & $\muR = \muF = \HT$/2, with  $\HT$ =  %$\Sigma_i^{N_{fs particle}}\, %\sqrt{p_\textrm{T,i}^2+m_i^2}$ \\
%Scale variations &  $\muR = \muF$ and \alphas in PS by factor of 0.5(2) \\
%QCD+EW &  tree-level EW ($\mathcal{O}(\alpha^3+\alphas %\alpha^3))$ added on top of  NLO QCD $\mathcal{O}(\alphas^2 \alpha + \alphas^3 \alpha) $ \\
%\hline\hline
%\end{tabular}
%}
%\end{center}

%\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{sidewaystable}
%\begin{center}
%\caption{\label{tab:mcconfig}
%The configurations used for the event generation of the \ttW processes.}
%\vspace{0.25cm}
%{\small
%\setlength\tabcolsep{1.5pt}
%\begin{tabular}{lllllll}
%\hline\hline
%Experiment & Generator & ME order & ME scale & Parton shower & PDF & Tune  \\
%%& (alternative) & (alternative) & & \\
%\hline
%ATLAS  & \textsc{Sherpa 2.2.8} & \textsc{MePs@Nlo} 0,1@NLO+2@LO & \, $\mu_R = \mu_F = H_\textrm{T}$/2 \,& \textsc{Sherpa} &  NNPDF3.0 NNLO & \textsc{Sherpa} default \\
%ATLAS & \textsc{MG5\_aMcAtNlo  2.3.3} & NLO & \, $\mu_R = \mu_F = H_\textrm{T}$/2 \, & \textsc{Pythia} 8.210 & NNPDF3.0 NLO & A14   \\
%CMS & \textsc{MG5\_aMcAtNlo 2.4.2} & NLO 0,1 jet @NLO + FxFx &   & \textsc{Pythia} 8.226 & NNPDF3.1 NLO  & CP5 \\
%\hline\hline
%\end{tabular}
%}
%\end{center}
%\end{sidewaystable}

%\begin{table}
%\footnotesize
%\begin{center}
%\caption{\label{tab:mcconfig} The configurations used for the event generation of the \ttW processes. Scale settings given in terms of $\mathrm{H_T} = \sum_{i=0}^{i=N}\sqrt{p_{T,i}^2+m_i^2}$, where N = number of final state particles.}
%\vspace{0.25cm}{
%\setlength\tabcolsep{6.pt}
%\renewcommand{\arraystretch}{1.5}
%\begin{tabular}{|l|l|l|l|}
%\hline\hline
%\bf{Experiment} & ATLAS & ATLAS & CMS \\ \hline
%\bf{Label} & ATLAS Sherpa 2.2.8 & ATLAS aMC@NLO & CMS aMC@NLO FxFx \\ \hline
%\bf{Process} & $\mathrm{t\bar{t}W}$ inclusive & $\mathrm{t\bar{t}W}$ inclusive & $\mathrm{t\bar{t} \ell \nu}$ \\ \hline
%\bf{Generator} & Sherpa 2.2.8\cite{Gleisberg:2008ta} & MG5\_aMcAtNlo v2.3.3\cite{madgraphamcNLO} & MG5\_aMcAtNlo v2.4.2 \\ \hline
%\bf{ME order} & 0,1@NLO+2@LO & NLO & 0,1 jet @NLO \\ \hline
%\bf{ME Scale} & $\mu_\mathrm{R}=\mu_\mathrm{F}=\mathrm{H}_T/2$ & $\mu_\mathrm{R}=\mu_\mathrm{F}=\mathrm{H}_T/2$ & Dynamical scale choice \cite{Frederix:2012ps,Catani:2001cc,Hamilton:2012np} \\ \hline
%\bf{Parton Shower} & Sherpa 2.2.8 & Pythia 8.210\cite{Sjostrand:2014zea} & Pythia 8.226\\ \hline
%\bf{Merging Scheme} & MEPs@NLO\cite{MEPs@NLO} & - & FxFx\cite{Frederix:2012ps} \\ \hline
%\bf{Merging Scale} & 30\,GeV & - & 42 GeV \\ \hline
%\bf{PDF} & NNPDF3.0 NNLO\cite{NNPDF3p0} & NNPDF3.0 NLO & NNPDF3.1 NLO\cite{NNPDF:2017mvq} \\ \hline
%\bf{Tune} & Sherpa default & A14 & CP5 \\ \hline
%\hline
%\end{tabular}
%}
%\end{center}
%\end{table}


%Josh update of the above for ATLAS FxFx

\begin{sidewaystable}
%\begin{table}
\footnotesize
\begin{center}
\caption{\label{tab:mcconfig} The configurations used for the event generation of the \ttW processes. Scale settings given in terms of $\HT = \sum_{i=0}^{i=N}\sqrt{p_{T,i}^2+m_i^2}$, where N = number of final state particles.}
\vspace{0.25cm}{
\setlength\tabcolsep{6.pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|l|l|l|}
\hline\hline
%\bf{Experiment} & ATLAS & ATLAS & ATLAS  \\ \hline
\bf{Label} & ATLAS Sherpa 2.2.10  & ATLAS Sherpa 2.2.10 QCD+EW & ATLAS aMC@NLO FxFx & ATLAS aMC@NLO   \\ \hline
% & ATLAS Sherpa 2.2.10 QCD+tree-level EW & & \\ \hline
\bf{Process} & $\mathrm{t\bar{t}W}$ inclusive & $\mathrm{t\bar{t}W}$ inclusive & $\mathrm{t\bar{t}W}$ inclusive & $\mathrm{t\bar{t}W}$ inclusive  \\ \hline
\bf{Generator} & Sherpa 2.2.10\cite{Sherpa} & Sherpa 2.2.10\cite{Sherpa} & MG5\_aMcAtNlo v2.9.3\cite{Alwall:2006yp} & MG5\_aMcAtNlo v2.3.3\cite{Alwall_2014}  \\ \hline
\bf{order of QCD ME } & 0,1@NLO+2@LO & 0,1@NLO+2@LO & 0,1@NLO  & NLO  \\ \hline
\bf{ME Scale} & $\muR=\muF=\HT/2$
 & $\muR=\muF=\HT/2$ & $\muR=\muF=\HT/2$ & $\muR=\muF=\HT/2$  \\ \hline
\bf{order of EW corrections} & - & $\alpha^3$,  $\alpha^{2}\alphas^{2}$, $\alpha^3\alphas$ & - & -\\ \hline
\bf{Parton Shower} & Sherpa 2.2.10 & Sherpa 2.2.10 & Pythia 8.245\cite{Sjostrand:2014zea} & Pythia 8.210\cite{Sjostrand:2014zea} \\ \hline
\bf{Merging Scheme} & MEPs@NLO\cite{Hoeche:2012yf} & MEPs@NLO\cite{Hoeche:2012yf} & FxFx\cite{Frederix:2012ps} & - \\ \hline
\bf{Merging Scale} & 30\,GeV & 30\,GeV & 30\,GeV & -  \\ \hline
\bf{PDF} & NNPDF3.0 NNLO\cite{NNPDF:2014otw} & NNPDF3.0 NNLO & NNPDF3.0 NLO & NNPDF3.0 NLO  \\ \hline
\bf{Tune} & Sherpa default & Sherpa default & A14\cite{ATL-PHYS-PUB-2014-021} & A14\cite{ATL-PHYS-PUB-2014-021}  \\ \hline
\bf{$\sigma_{tot}$\footnote{ $\sigma_{tot}$=600.8~fb from YR4 is used for all samples in the generator comparisons in section\,\ref{sec:ttw_gen} } & 597.0~fb & 614.7~fb & 613 fb & 548~fb  \\ \hline
\hline
\end{tabular}
}
\end{center}
\end{sidewaystable}
%\end{table}



%\cite{ATL-PHYS-PUB-2014-021}
%CP5\cite{Sirunyan:2019dfx}
% Finally, the uncertainty due to the choice of PDF set is evaluated using the PDF4LHC15 prescription.

\subsection{Object reconstruction, fiducial volume and observables}
\label{sec:ttw_fid}
Object and event selection is defined at particle-level that closely matches the detector-level described in reference~\cite{ATLAS-CONF-2019-045} (ATLAS) and~\cite{CMS-HIG-19-008} (CMS). %and was defined together with CMS as a common phase space.
Jets are reconstructed from all stable final state particles with a mean lifetime of $\tau \gr 3\times 10^{-11}$~s (but excluding leptons and neutrinos from the top quark decay chain), using the anti-$k_t$ algorithm with a radius parameter of $R=0.4$.
Jets are required to satisfy \pt  \gr 25 GeV and $|\eta|$ \less 2.5.
Jets that are matched to a $b$-hadron\footnote{no \pt cut is applied} by ghost matching~\cite{Cacciari:2008gn} are referred to as $b$-jets.
Electrons and muons, referred to as light leptons $\ell$, are required to be separated from selected jets by $\Delta R\gr0.4$ and are otherwise removed.
Hadronically decaying $\tau$ leptons are required to satisfy \pt\gr 25 GeV and $|\eta| $\less 2.5.
Events are selected with exactly two light leptons. The four-momentum of the bare leptons from top quark decay are modified (”dressed”) by adding the four-momenta of all radiated photons within a cone of size $\Delta R = 0.1$.
Leptons are required to have $|\eta|$\less 2.5 and \pt\gr25(20) GeV for leading $\ell_0$ (subleading $\ell_1$) lepton (\pt ordered).
Leptons are required to have same charge, targeting the semi-leptonic $\mathrm{t\bar{t}}$ decay and leptonic $W$ decay.

%Events separated by Hadronic tau decays Hadronically decaying $\tau$ lepton
Events with at least 3 jets and at least one of them being a $b$-jet are considered in the fiducial volume. The object definition and event selection is summarised in Tables\,\ref{tab:ttWobjects} and \ref{tab:ttWeventselection}. 
%Events with at least 3 jets and least one $b$-jet are considered in the fiducial volume.
%The acceptance for events passing this selection is $A_X^{\geq1b\geq3j}=1.XX\times10^{-2}$ for \textsc{Sherpa} and 1.ZZ$\times10^{-2}$ for \textsc{MadGraph5\_aMC@NLO} correspondingly.
These are then split into five regions, categorized by the number of jets of any flavour (three or  $\geq$4), $N_{b-\mathrm{jets}}$ (one or $\geq$2) as well as the presence of hadronically decaying $\tau$ lepton, as summarised in Table~\ref{tab:ttWregions}.

\begin{table}
\begin{center}
\caption{\label{tab:ttWobjects}
The object reconstruction used in the Rivet analysis of the \ttW processes.}
%with lifetime $\tau > 3 \cdot 10^{-11}$ s
\vspace{0.25cm}
{\small
\setlength\tabcolsep{1.5pt}
\begin{tabular}{| l |}
\hline
\textbf{Object reconstruction and selection}\\
%& (alternative) & (alternative) & & \\
\hline
\hline
Jets: build from stable final state particles with anti-k$_t$ algorithm with  radius R = 0.4 \\
the prompt "dressed" leptons and neutrinos are vetoed from jet \\
 $b$-jets: Jets ghost matched to $B$-hadrons with \pt $>$ 5 GeV \\
Jets and $b$-Jets:  \pt  \gr 25 GeV and $|\eta|$ \less 2.5 \\
\hline
light leptons (electrons and muons) dressed with photons within $\Delta R <$ 0.1 \\
Overlap removal: remove light lepton if $ \Delta R(jet, lepton) < 0.4 $\\
leptons: $|\eta|$\less 2.5 and \pt\gr 25(20) GeV for leading  (subleading) lepton\\
hadronicaly decaying $\tau$ leptons (before decay):  \pt  \gr 25 GeV and $|\eta|$ \less 2.5 \\

%2 & $N_{b-\mathrm{jets}}\geq$2,   $N_{\mathrm{jets}}\geq$4, 0-$\tau_{had}$ \\
%3 & $N_{b-\mathrm{jets}}=$1,  $N_{\mathrm{jets}}$=3 , 0-$\tau_{had}$ \\
%4 & $N_{b-\mathrm{jets}}\geq$2, $N_{\mathrm{jets}}$=3, 0-$\tau_{had}$ \\
%5 & $N_{b-\mathrm{jets}}\geq$1, $N_{\mathrm{jets}}\geq$3 , 1-$\tau_{had}$\\
%\hline\hline
%\textbf{Event selection}\\
%\hline
%exactly 2 leptons with same charge \\
%$N_{\mathrm{jets}}\geq$4 \\
%no hadronic $\tau$ \\
%$N_{b-\mathrm{jets}}=1$ or $N_{b-\mathrm{jets}}\geq$2 \\
%\hline
\hline
\end{tabular}
}
%\caption{Object and event selection defined at particle-level to closely match the detector-level  selections described in ATLAS-CONF-2019-045 }
\end{center}
\end{table}



\begin{table}
\begin{center}
\caption{\label{tab:ttWeventselection}
The event selection used in the Rivet analysis for the \ttW processes. $N_{\mathrm{jets}}$ refers to all jets independent of jet flavour, i.e. $b$-jets are included.}
\vspace{0.25cm}
{\small
%\setlength\tabcolsep{1.5pt}
%\begin{tabular}{l}
%\hline\hline
%Event Selection and Region definition \\
%%& (alternative) & (alternative) & & \\
%exactly 2 leptons with same charge \\
%$N_{\mathrm{jets}}\geq$3 \\
%$N_{b-\mathrm{jets}}\geq$1 \\
%\hline \hline
%\end{tabular}
%Region definition \\
\begin{tabular}{l}
\hline
\hline
\textbf{Event selection for 2$\ell$SS}\\
\hline
exactly 2 leptons with same charge  \\
$N_{\mathrm{jets}}\geq$3 \\
%no hadronic $\tau$ \\
 $N_{b-\mathrm{jets}}\geq$1 \\
\hline
\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{\label{tab:ttWregions}
The  region definitions used in the Rivet analysis for the \ttW processes.}
\vspace{0.25cm}
{\small
%\textbf{Region definition}\\
\begin{tabular}{l|l}
\hline
\hline
\textbf{Region} & \textbf{Selection} \\ \hline
1  & $N_{b-\mathrm{jets}}=$1, $N_{\mathrm{jets}}\geq$4 , 0-$\tau_{had}$ \\
2 & $N_{b-\mathrm{jets}}\geq$2,   $N_{\mathrm{jets}}\geq$4, 0-$\tau_{had}$ \\
3 & $N_{b-\mathrm{jets}}=$1,  $N_{\mathrm{jets}}$=3 , 0-$\tau_{had}$ \\
4 & $N_{b-\mathrm{jets}}\geq$2, $N_{\mathrm{jets}}$=3, 0-$\tau_{had}$ \\
5 & $N_{b-\mathrm{jets}}\geq$1, $N_{\mathrm{jets}}\geq$3 , 1-$\tau_{had}$\\
\hline
\hline
\end{tabular}
}
\end{center}
\end{table}

The definitions of the regions are motivated by the $t\bar{t}H$ Multilepton analysis strategy.
Regions 1 and 2 corresponds to the signal regions\footnote{slightly different then in ref.~\cite{ATLAS-CONF-2019-045}, in order to define a common selection with the CMS Collaboration.} and Regions 3 and 4 are used as control regions in the 2$\ell$ same-sign  0-$\tau_{had}$ $t\bar{t}H$ channel.
Definition of Region 5 is closely followed\footnote{requirement on jet multiplicity is relaxed.} by the selections in the 2$\ell$ same-sign 1-$\tau_{had}$ $t\bar{t}H$ channel.

%The event selection requirements are summarized in Table~\ref{}.
%defined by 5 jets \& 3 b-jets or >=6jets \& >=4 b-jets.

%\input{Tex/systematics.tex}


%$N_{jets}$, $N_{b-jets}$,  $HT^{\text{jets}}$, leading $b$-jet $p_T$ Leading lepton $p_T$, $|\Delta \phi _{\ell \ell }|$, $\Delta R _{\ell \ell }$, $max |\eta _l|$
\begin{table}[]
\begin{center}
\caption{\label{tab:ttw_varlist}
The list of the validation variables for the comparison of the \ttW generators. The leptons $\ell$ and $b$-jets are ordered in \pt - leading correspond to highest \pt. }
\vspace{0.25cm}
{\small
\setlength\tabcolsep{1.5pt}
\begin{tabular}{l|l|c}
\hline\hline
Variable & Description & Regions \\ \hline
$N_{jets}$   &     Jet multiplicity        &      1,2,5   \\ %\hline
 $N_{b-jets}$       &     Number of  $b$-jets       &   1,2,5      \\ %\hline
$\HT^{\text{jets}}$      & Scalar sum of transverse momentum of all jets in the event         &  1,2,3,4       \\ %\hline
$\pt^{b0}$       &      Leading $b$-jet transverse momentum       &   1,2      \\ %\hline
 $p_T^{\ell 0}$      &   Leading lepton transverse momentum           &     1,2,5    \\ %\hline
$\Delta R _{ \ell 0\mathrm{jets} }$      &     Minimum angular separation between the leading lepton and the nearest jet         &  1,2       \\ %\hline
$\Delta R _{\ell 0\ell1 }$      &       Angular distance between the two leptons      &    1,2,5    \\ %\hline
$max |\eta _{\ell}|$      &    Value of the highest lepton's pseudorapidity in the event        &     1,2    \\ %\hline
%    $\Delta \phi _{\ell \ell }$    &    Azimuthal separation between the leptons         & 1,2    \\
    \hline\hline
\end{tabular}
}
\end{center}
\end{table}
The list of variables for the comparison of the \ttW generators presented in this note are summarised in Table~\ref{tab:ttw_varlist}.
\clearpage
\subsection{Results}
%Distribution of the angular distance between the two leptons (top), maximum between lepton $|\eta_{\ell 0}|$ and $|\eta_{\ell 1}|$ (centre), azimuthal separation between the leptons $\Delta \phi _{\ell \ell }$ (bottom) , for the Region 1 with 1$b$-jet (left) and Region 2 with 2$b$-jets (right) selection requiring four and more jets.

%The samples  \textsc{Sherpa} \ttW  sample is compared to its radiation uncertainty variations and the alternative generator.
The samples described in Table~\ref{tab:mcconfig} are compared in the following. 
The ratio plots show the ratios of the all MC samples with respect to \textsc{Sherpa}, the shaded band represents scale variations.  %for ATLAS (blue) and \textsc{aMC@NLO FxFx} for CMS (red).
The same set of distributions are presented twice with different focus: in Sect.\,\ref{sec:ttw_shape}   shapes  are compared and in Sect.\,\ref{sec:ttw_gen}   acceptance effects are studied.  %as all distributions are scaled to the Yellow Report 4~\cite{YR4} cross section or the generator cross section for the sample including EW corrections. % (taken directly from generation - i.e. not including any correction factors).

\subsubsection{Shape comparison}
\label{sec:ttw_shape}
In the following shape agreement between nominal and alternative generators will be presented, i.e. the distributions are normalised to the integral.
%$N_{b-\mathrm{jets}}=$

%Sizeable discrepancies in the modelling of jet kinematics can be seen between the \textsc{Sherpa} \ttW and \textsc{MadGraph5\_aMC@NLO} generators in the $N_{b-\mathrm{jets}}$=1 regions, while in the $N_{b-\mathrm{jets}}\geq$2 regions the difference is reduced, as illustrated in

The modelling of jet kinematics are presented on Figure~\ref{ttW:4j12b}  for the high (Regions 1 and 2) and low (Regions 3 and 4) jet multiplicities. Significant differences between \sherpa and  \amc are observed which are not present for \amc FxFx. 
%Differences in distributions of $b$-jet kinematics follow a similar trend - sizeable discrepancies in the $N_{b-\mathrm{jets}}$=1 regions and agreement within scale uncertainties in the $N_{b-\mathrm{jets}}\geq$2 regions, as presented on Figures~\ref{ttW:4jbinfo} for Regions 1 and 2.


\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_nJets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_nJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_HT_jets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_HT_jets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_2_HT_jets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_3_HT_jets.pdf}\\
  \caption{Distribution of the jet multiplicities (top) and the scalar sum of jets transverse momentum, $H_{\mathrm{T}}^{\text{jets}}$ (middle), for the Region 1 with $N_{b-\mathrm{jets}}=$1 (left) and Region 2 with  $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets, and  for the Region 3 $N_{b-\mathrm{jets}}$ = 1 (bottom, left) and Region 4 with $N_{b-\mathrm{jets}}\geq$2 (bottom, right) selection requiring exactly three jets.  \label{ttW:4j12b}\label{ttW:3j12b}}
\end{figure}


%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_2_HT_jets.pdf}
%\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_3_HT_jets.pdf}\\
%  \caption{Distribution of the scalar sum of jets transverse momentum, $H_{\mathrm{T}}^{\text{jets}}$, for the Region 3 $N_{b-\mathrm{jets}}$ = 1 (left) and Region 4 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring exactly three jets.  \label{ttW:3j12b}}
%\end{figure}


\begin{figure}[!htb]
\centering
%\includegraphics[width=0.45\textwidth]{Plots/ttw/FxFx/dummy}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_nBtagJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_Bjet_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_Bjet_Pt_0.pdf}\\
  \caption{Distribution of the $b$-jet multiplicities (top) and the leading $b$-jet transverse momentum (bottom), for the Region 1 with $N_{b-\mathrm{jets}}$=1 (left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets.  \label{ttW:4jbinfo}}
\end{figure}

%Good agreement of the single lepton kinematics can be seen between nominal and alternative generators for the $N_{b-\mathrm{jets}}\geq$2 regions, as shown on the right of
The lepton kinematics distributions are shown on Figure~\ref{ttW:lep_kin} representing Region 2. Overall, good agreement between all predictions is observed. 
%Similar behaviour is also seen in Region 4.
%While there is an offset of the order of 10\%  between nominal and alternative generators for 1$b$-jet selections, as presented in the left of Figures~\ref{ttW:lep_kin} (Region 1 showed, while similar trend seen in Region 3 as well).

%Sizeable differences in shapes between nominal and alternative generators are observed for the distributions involving correlations between the two leptons.
The distributions of the angular distance between the two leptons and the maximum of lepton's pseudorapidity  separation between the leptons are presented in Figure~\ref{ttW:ll_kin} for Region 1 on the right and Region 2 on the left. Good agreement of the distributions is observed except for \amc. 
%Similar behaviour is also seen in Regions 3 and 4.
%As was observed for single lepton kinematics, difference in 1$b$-jet selections is increased wrt to $\geq2b$-jets selection.
%Distributions are presented for $\geq2N_{b-jets},\geq4N_{jets}$ region, while similar behaviour seen in all other regions as well.

Distributions of the jet multiplicity, number of $b$-jets, the leading lepton transverse momentum and the angular distance between the two leptons  $\Delta R _{\ell 0\ell1 }$ for the Region 5 with $N_{\tau_\mathrm{had}}$ = 1 selection are presented in Figure ~\ref{ttW:tauR_kin}. In contrast to all other comparisons, the jet multiplicity prediction of \amc with FxFX differs most from the other predictions in this region.
%The difference observed between nominal and alternative generators for high jet multiplicities, at the edge of the scale variation uncertainty band.
%The distribution of $N_{b-\mathrm{jets}}$ is in agreement for $N_{b-\mathrm{jets}}$ = 2, while a sizeable difference is observed for $N_{b-\mathrm{jets}} = 1$, which is similar to the $N_{\tau_\mathrm{had}}$ = 0 selections.
%Lepton kinematic distributions show differences in shapes between the nominal and alternative generator.

\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_lep_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_lep_Pt_0.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_min_DRl0j.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_min_DRl0j.pdf}\\
  \caption{Distribution of the leading lepton transverse momentum (top) and the minimum angular separation between the leading lepton and the nearest jet (bottom), for the Region 1 with $N_{b-\mathrm{jets}}$=1(left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2(right) selection requiring four and more jets.
  \label{ttW:lep_kin}}
\end{figure}

\begin{figure}[!htb]
\centering
	% \hspace{25mm} $DRl_0l_1$  \hspace{20mm} $max|\eta^{\ell\ell}|$\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_DRll01.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_DRll01.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_0_maxEta_ll.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_1_maxEta_ll.pdf}\\
%\includegraphics[width=0.45\textwidth]{Plots/ttw/FxFx/shape/c_Region_0_lep_dPhi}
%\includegraphics[width=0.45\textwidth]{Plots/ttw/FxFx/shape/c_Region_1_lep_dPhi}
  \caption{Distribution of the angular distance between the two leptons (top), maximum between lepton $|\eta_{\ell 0}|$ and $|\eta_{\ell 1}|$(bottom) , for the Region 1 with $N_{b-\mathrm{jets}}$=1 (left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2(right) selection requiring four and more jets.
  % (centre), azimuthal separation between the leptons $\Delta \phi _{\ell \ell }$ 
   \label{ttW:ll_kin}}
\end{figure}
%



\begin{figure}[!htb]
\centering

\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_4_nJets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_4_nBtagJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_4_lep_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_n/c_Region_4_DRll01.pdf}\\
  \caption{Distribution of the the jet multiplicity, number of $b$-jets, the leading lepton transverse momentum and the angular distance between the two leptons  $\Delta R _{\ell \ell }$ for the Region 5 with 1$\tau_{had}$ selection.
   \label{ttW:tauR_kin}}
\end{figure}
%

\clearpage
\newpage

%
%
%
%%
%
%
\subsubsection{Comparisons of predictions including acceptance effects}
\label{sec:ttw_gen}

In the following section a comparison of the generators will be given in the fiducial phase space, i.e. the predicted distributions include acceptance effects. 
%Some difference is observed in $\sigma_{fid}^{gen}=A_X^{gen}\times \sigma_{tot}^{gen}$ , where $A_X^{gen}$ is the acceptance factor of particular region, $\sigma_{tot}^{gen}$ is the total generator cross section times $k$-factor to match Yellow Report cross section value.
%The generator cross sections are $\sigma_{tot}^{Sherpa}=$589~fb for Sherpa and $\sigma_{tot}^{MG5\_aMcAtNlo}=548$~fb  for  ATLAS MG5\_aMcAtNlo sample.
For this comparison,  all  distributions without EW corrections are normalised to  match the total cross section value of $\sigma_{tot}^{YR4}=$600.8~fb as given in the Yellow Report 4 \cite{YR4} for predictions without EW corrections. The distributions of Sherpa QCD+EW which are normalised to their generator cross section of 614.7 fb. 
%The fiducial cross sections of the five regions defined in Section~\ref{sec:ttw_fid} are presented on Figure~\ref{ttW:fid_xs}.
The same set of distribution discussed in Section~\ref{sec:ttw_shape} are presented. %normalised to the fiducial cross section. %in  Figures~\ref{fig:den_4j12b}-\ref{fig:den_tauR_kin}.
In all distribution, a significant increase of scale uncertainties is observed, reaching up to 50\% at high jet multiplicity. 
The observables related to jet multiplicity and \HT show   similar trends as in the shape comparisons, see Figure~\ref{fig:den_3j12b}. Only the discrepancy of the jet multiplicity prediction in \amc FxFx is significantly enhanced. 
%\begin{figure}[!htb]
%\centering
%%\includegraphics[width=0.55\textwidth]{Plots/ttw/FxFx/generator/acc_7f}
%  \caption{The fiducial cross sections, $\sigma_{fid}^{gen}=A_X^{gen}\times \sigma_{tot}^{gen}$,  of the five regions for $ttW$ analysis. \label{ttW:fid_xs}}
%\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_nJets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_nJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_HT_jets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_HT_jets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_2_HT_jets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_3_HT_jets.pdf}\\
  \caption{Distribution of the jet multiplicities (top) and the scalar sum of jets transverse momentum, $H_\text{T}^{\text{jets}}$ (middle), for the Region 1 with $N_{b-\mathrm{jets}}$=1 (middle, left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2 (middle, right) selection requiring four and more jets. 
   $H_\text{T}^{\text{jets}}$, for the Region 3 with $N_{b-\mathrm{jets}}$=1 (bottom, left) and Region 4 with $N_{b-\mathrm{jets}}\geq$2 (bottom, right) selection requiring exactly three jets.
  All distributions are normalised to YR4 cross section of 600.8 fb. 
  \label{fig:den_3j12b}
  \label{fig:den_4j12b}}
\end{figure}


%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_2_HT_jets.pdf}
%\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_3_HT_jets.pdf}\\
%  \caption{Distribution of the scalar sum of jets transverse momentum, $HT^{\text{jets}}$, for the Region 3 with $N_{b-\mathrm{jets}}$=1 (left) and Region 4 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring exactly three jets. All distributions are normalised to YR4 cross section of 600.8 fb.  \label{ttW:den_3j12b}}
%\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_nBtagJets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_nBtagJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_Bjet_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_Bjet_Pt_0.pdf}\\
  \caption{Distribution of the $b$-jet multiplicities (top) and the leading $b$-jet transverse momentum (bottom), for the Region 1 with $N_{b-\mathrm{jets}}$=1 (left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets. All distributions are normalised to YR4 cross section of 600.8 fb.  \label{ttW:den_4jbinfo}}
\end{figure}



\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_lep_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_lep_Pt_0.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_min_DRl0j.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_min_DRl0j.pdf}\\
  \caption{Distribution of the leading lepton transverse momentum (top) and the minimum angular separation between the leading lepton and the nearest jet (bottom), for the Region 1 with $N_{b-\mathrm{jets}}$=1 (left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets. All distributions are normalised to YR4 cross section of 600.8 fb. 
  \label{ttW:den_lep_kin}}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_DRll01.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_DRll01.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_0_maxEta_ll.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_1_maxEta_ll.pdf}\\
%\includegraphics[width=0.45\textwidth]{Plots/ttw/FxFx/r3_v32yr4_NN1_f/c_Region_0_lep_dPhi}
%\includegraphics[width=0.45\textwidth]{Plots/ttw/FxFx/r3_v32yr4_NN1_f/c_Region_1_lep_dPhi}
  \caption{Distribution of the angular distance between the two leptons (top), maximum between lepton $|\eta_{\ell 0}|$ and $|\eta_{\ell 1}|$ (centre), %azimuthal separation between the leptons $\Delta \phi _{\ell \ell }$ (bottom) ,
   for the Region 1 with $N_{b-\mathrm{jets}}$=1 (left) and Region 2 with $N_{b-\mathrm{jets}}\geq$2 (right) selection requiring four and more jets. All distributions are normalised to YR4 cross section of 600.8 fb. 
   \label{ttW:den_ll_kin}}
\end{figure}
%



\begin{figure}[!htb]
\centering
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_4_nJets.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_4_nBtagJets.pdf}\\
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_4_lep_Pt_0.pdf}
\includegraphics[width=0.45\textwidth]{Plots/ttW/FxFx/r3_v32yr4_NN1_f/c_Region_4_DRll01.pdf}\\
  \caption{Distribution of the the jet multiplicity, number of $b$-jets, the leading lepton transverse momentum and the angular distance between the two leptons  $\Delta R _{\ell \ell }$ for the Region 5 with 1$\tau_{had}$ selection. All distributions are normalised to YR4 cross section of 600.8 fb. 
   \label{fig:den_tauR_kin}}
\end{figure}
%
\include{FxFxPlots}
\subsection{Conclusion}
The \ttW preditions of \sherpa and \amc with different settings have been compared in regions and observables relevant for the  measurement of \ttH in the multi-lepton final state. The normalised distributions sensitive to shape differences have  very small scale uncertainties, below 10\% in most of the phase space while these scale uncertainties are significant when the acceptance effects are included, i.e. the distributions are normalised to the \ttW cross section. The inclusion of tree-level EW effects only causes minor shape effects but can lead to up to 20\% difference in cross section at high jet multiplicity. As expected  including the FxFx algorithm into the \amc prediction leads to significant effects in all regions, especially at low \HT. Overall,  the differences between the different model predictions are mostly within the scale uncertainty band except at the edges of the phase space.\\
These distributions will be used for future comparisons with CMS to derive a theory uncertainty model for a combination of the expected measurement results based on the full Run2 data set.

==> Tex/ttbb_approved_ATLAS.tex <==
%-------------------------------------------------------------------------------
\section{Comparisons of Monte Carlo predictions for the \ttbb process}
\label{sec:ttbb}


%-------------------------------------------------------------------------------

In the following section \ttbb background predictions  used by ATLAS in published and future analyses of \ttHbb are compared.  Several MC generator implementations where \ttbb matrix elements are calculated at NLO with massive $b$-quarks\footnote{"quarks" refers to both quarks and anti-quarks} using the four-flavour (4FS) PDF sets  \cite{ttbbtheo1,ttbbtheo2} are used. 
The implementation in the \powhegboxres framework~\cite{Jezo:2015aia, Jezo:2018yaf}  matched to \pythiaa~\cite{Sjostrand:2014zea} for parton shower, hadronization, multi-parton interaction and beam remnant, referred to as parton shower generator for short, is used as nominal prediction in ATLAS physics analyses based on the full Run-2 data set and referred to as  PP8 \ttbb in the following. 
% Removed! However, the experiments use slightly different parameter settings both in the \powhegboxres  calculation and in \pythiaa as will be described in the following.

 In order to estimate systematic uncertainties ATLAS considers predictions with  different settings of the   \powhegboxres internal parameter \bornzero which regulates the splitting into the finite and the  singular part of the real emission in the NLO calculation. In addition,  set-ups of \powhegboxres  matched to  different parton shower generators  are considered.  %, changes to dipole recoil 
 %from the default value 2 as in \cite{Jezo} to  5  as recommended for \ttbar  \cite{powheg} and recently also for \ttbb. Furthermore, 
 % in the \pythiaa parton shower  %by switching  to dipole recoil in  \pythiaa 
% and  finally, matching to  \herwiga~\cite{Herwig7} as parton shower generator. 
 Details of these samples are given in~\cite{ttbbpubnote}. The dependence on the particular choice of generator and the NLO matching algorithm is studied by comparing to predictions of  \sherpa 2.2.10~\cite{Sherpa,Cascioli:2013era, Cascioli:2011va}.
%ATLAS varies    the matching parameter $h_{bzd}$ in  \powhegboxres and studies matching to a varied \pythiaa parton shower set-up and  to  \herwiga \cite{Herwig7} as described in \cite{ttbbpubnote}.  
  
  %CMS varies the matching parameter $h_{\text{damp}}$ in   \powhegboxres.
   %The dependence on  the NLO matching algorithm is studied by comparing to predictions of  \amc.
 
  Finally, the uncertainties on the renormalization and factorization scales, \muR and \muF, are estimated by varying them simultaneously in the matrix element (ME) by a factor 0.5 (2) around the nominal value. The dependence on  the value of the strong coupling constant, 
    \alphas,  in the initial and final-state radiation simulation of the parton shower (PS ISR, PS FSR) is estimated  by varying them independently also by a factor two up and down, i.e. one scale   is changed at a time while keeping the other parameters at their nominal value. %The systematic uncertainty estimates due to scale variations are summarised in Table~\ref{tab:tttbbvariations}.
  %PDF uncertainties are  are  neglected in the studies presented here due to the smallness of the effect. 

The first Run-2 \ttHbb analysis of ATLAS~\cite{ttHbb} used a partial data set  and based the background predictions on  inclusive \ttbar production with the  matrix element calculated at NLO QCD  with \powheg~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Campbell:2014kua,Jezo:2015aia} employing a 5FS PDF and additional partons including $b$-quarks  produced by the \pythiaa parton shower. % In order to examine the effects introduced by changing the nominal generator, comparisons between these old and the new nominal predictions are provided. 
The first full Run-2 \ttHbb  analysis ~\cite{ttHbbRun2} changed the nominal generator to PP8 \ttbb. However, it used a different set-up compared to the future analyses:    the  renormalization scale was set to two times the renormalization scale  recommended to date by the LHC Higgs WG and  %Table\,\ref{tab:ttbbscalechoices}  
the difference between  the inclusive  \ttbar samples was used  to derive relative uncertainties which are attached to the nominal PP8 \ttbb sample.
    
The studies presented here provide comparisons of the   \ttbb PP8  predictions, the  variations considered to estimate uncertainties and comparisons to the  predictions used in the first full Run-2 \ttHbb analyses. All comparisons are performed using stable final state particles in a fiducial phase space similar to the experimental measurements implemented in a dedicated routine in  the \rivet analysis toolkit~\cite{rivet}.

%with the aim to show modelling differences  and to develop a scheme for systematic uncertainty estimate to be used in a posssible future combination of the results. 
%We demonstrate the variations considered by the two experiments to estimate the systematic uncertainty on the predictions. 
%The predictions are compared using observables and fiducial phase spaces similar to the ones used in the different \ttHbb analyses which varies slightly between experiments and  between publications of one experiment.
The section is organised as follows: in Sec.\,\ref{sec:samples} describes the samples used for the comparison and the technical set-up of their generation. Section\,\ref{sec:rivet} describes the observables and the fiducial phase space used for the comparison and finally, Sec.\,\ref{sec:results} displays the resulting comparisons.

\subsection{MC generator set-ups}\label{sec:samples}
%Different Monte Carlo (MC) generators are compared in this study, and results for two of these are available from both ATLAS and CMS.
The set-ups used to generate \ttbb predictions with  \powhegboxres, \powheg,  \amc  and \sherpa  are described in the following. The generator configurations and version numbers are summarised in Table~\ref{tab:ttbbsamples} and their scale settings are given in Table~\ref{tab:ttbbscalechoices}. The systematic uncertainty estimates due to scale variations are summarised in Table~\ref{tab:ttbbvariations}.

The $b$-quark mass  is set to \SI{4.75}{\GeV} for \sherpa and to  \SI{4.95}{\GeV} for  all other ATLAS samples.  The top quark mass is assumed to be \SI{172.5}{\GeV}. The decay of the top quark is calculated by the corresponding generators  (\powheg, \sherpa) respecting the spin correlation. The PDF sets are selected from the NNPDF3.0 family for all samples. The  \powhegboxres and \powheg samples use EvtGen \cite{evtgen} for simulation of the $B$-hadron decays. 

%Systematic variations are listed in Tab.~\ref{tab:tttbbvariations}.

\begin{description}
\item[\powhegboxres \ttbb samples:]~\\
 Nominal \ttbb predictions are calculated using the \powhegboxres framework at NLO with massive $b$-quarks~\cite{Jezo:2018yaf}  with the "4FS NLO as 0118" PDF sets. The \powhegboxres internal parameter $h_{\text{bzd}}$ is set to 5. The renormalization scale  is set to the geometric average of the transverse mass of top- and $b$-quarks  defined as %$m_{\text{T},\text{i}} = \sqrt{m^2_{\text{i}} + p^2_{\text{T},\text{i}}}$, where $p_{\text{T},\text{i}}$ 
$m_{\text{T},i} = \sqrt{m^2_i + p^2_{\text{T},i}}$, where $m_i$ refers to the  mass, $p_{\text{T},i}$
to the transverse momentum and $i$  to the top or $b$-quark. %in the \ttbar center-of-mass reference frame.
%$\mu_R=\sqrt[4]{m_{\text{T},\text{t}}\times m_{\text{T},\overline{\text{t}}}\times m_{\text{T},\text{b}}\times m_{\text{T},\overline{\text{b}}}}$ 
The factorization scale is related to the average of the transverse mass of the outgoing partons in the matrix element calculation, see Table~\ref{tab:ttbbscalechoices}.
%It is set to a factor two lower in CMS compared to ATLAS as detailed in Table~\ref{tab:ttbbscalechoices}.
%Here the process described in Ref.~\cite{Jezo:2018yaf} is followed.
The \pythiaa parameters for parton shower and hadronization modelling are set to the A14~\cite{ATL-PHYS-PUB-2014-021} tune.
These samples are referred to as PP8 \ttbb samples.

For the $h_{\text{bzd}}$ variation,  the parameter $h_{\text{bzd}}$ is set to 2 in the \powhegboxres framework.
For  the parton shower variations, the set of LHE files  which store the results of the matrix element calculation by \powhegboxres for the PP8 sample  are used and matched to a different parton shower prediction. For the  prediction with 
 \pythiaa dipole shower only the treatment of the  recoil of the radiated parton  in the  shower  is changed and all other parameters are kept as the A14 tuned values. Another sample is produced where \herwiga is used with the default tune provided with this generator version. 



The \powhegboxres\ \ttbb\ samples were calculated using a special option where virtual corrections are switched off and then reweighted with virtual corrections switched on\footnote{steered via "for\_reweight 1"}.


\item[\sherpa \ttbb samples:]~\\
A \sherpa \ttbb sample was generated using \sherpa version~2.2.10~\cite{Sherpa,Cascioli:2013era, Cascioli:2011va}.
The \ttbb matrix elements were calculated with massive $b$-quarks at NLO, using the \textsc{COMIX}~\cite{Gleisberg:2008fv} and \openloops~\cite{Cascioli:2011va} matrix element generators, and merged with the Sherpa parton shower, tuned by the authors~\cite{Schumann:2007mg}.
%The 4FS PDF set NNPDF3.0 with $\alphas=0.118$ is used.% and the b-quark mass is set to \SI{4.75}{GeV}.
The same renormalization and factorization scales and PDFs are used as for the PP8 \ttbb prediction.


 

%A sample was generated by CMS using  \amc  version~2.4.2 with the xxx scales. The matrix element calculation is using the same PDF and is matched to \pythiaa with the same tune as the nominal CMS PP8 sample.
% and set to half of the sum of the transverse masses for ATLAS and to a quarter  of the sum for CMS, as detailed in Table~\ref{tab:ttbbscalechoices}.  The parton shower and the hadronization were modelled by \pythia~8.210~\cite{PhysRevD.78.014026} with the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} for ATLAS and by \pythia~8.230~\cite{Sjostrand:2014zea} with the CP5 set of tuned parameters~\cite{Sirunyan:2019dfx} for CMS, respectively. These samples are referred to as PP8 \ttbb samples.
%are used as nominal in the most recent \ttHbb analyses by both experiments and 


% $\mu_F=\frac{1}{2} (m_{\text{T},\text{t}}+m_{\text{T},\overline{\text{t}}}+m_{\text{T},\text{b}}+m_{\text{T},\overline{\text{b}}}+m_{\text{T},\text{g}})$

%The \hdamp parameter was set to the sum of the transverse masses of the top and bottom quark and anti-quarks for ATLAS \todo{correct? table states 1.5mtop} and to 1.379 times the top quark mass for CMS, where the top quark mass is assumed to be \SI{172.5}{\GeV}.This sample is referred to as PP8 \ttbb sample.


% $\mu_R=\sqrt[4]{m_{\text{T},\text{t}}\times m_{\text{T},\overline{\text{t}}}\times m_{\text{T},\text{b}}\times m_{\text{T},\overline{\text{b}}}}$ and $\mu_F=\HT/2$.

%A \sherpa \ttbar sample was generated with \sherpa version~2.2.1 with the \textsc{MEPS}@NLO (multi-leg) setup using the \textsc{MEPS}@NLO prescription~\cite{Hoeche:2012yf}, interfaced with \openloops. It provides NLO accuracy for up to one additional parton and LO accuracy for up to four additional partons. The NNPDF3.0 NNLO PDF set is used with a five-flavour scheme and both renormalization and factorization scales are set to $\sqrt{0.5\times(m_{T,t}^2+m_{T,\bar{t}}^2)}$. 

%CMS generated another \ttbb sample  with \amc version~2.4.2, using the 4FS PDF set NNPDF3.1 with $\alphas=0.118$ and matched to Pythia~8.230 with the CP5 tune. % and a b-quark mass of \SI{4.75}{GeV}.
%The scales were set to $\mu_R=$ and $\mu_F=$ \todo{?}.
%The parton shower and hadronization is modeled by Pythia~8.230 with the CP5 tune.

%Both the PP8 \ttbb, the \sherpa \ttbb, and the \amc \ttbb samples describe the additional \bbbar-pair with NLO precision in QCD, taking into account the b-quark mass.

\item[Inclusive  \ttbar samples:]~\\
The inclusive \ttbar samples are generated with the \powheg v2 NLO event generator~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Campbell:2014kua,Jezo:2015aia} and \amc  using a five-flavour (5FS) PDF set. %and   matched to \pythia such that the additional \bbbar-pair is described by the parton shower. 
The renormalization and factorization scales were set to the average transverse mass of the top quark and antiquark. 

For the \powheg samples, the \hdamp parameter\footnote{The \hdamp parameter controls the \pt of the first additional emission beyond the leading-order Feynman diagram in the PS and
therefore regulates the high-\pt emission against which the \ttbar system recoils.} was set to the 1.5 times the top quark mass. One sample is generated with the parton shower and hadronization modeled by \pythiaa with the same versions and settings as for the PP8 \ttbb sample above. Another sample is generated using \herwiga for the parton shower and hadronization. 
 %These samples were used as the nominal background estimate in  $\ttH(\bbbar)$ analyses based on 36 \ifb \cite{atlastthbb, cmstthbb} \todo{check cms citation. Were was this used/}
The \powheg \ttbar samples are filtered to contain only semi-leptonic and dileptonic \ttbar decays with exactly one or two leptons, respectively, within the fiducial volume as defined further below.
These samples are referred to as PP8 \ttbar and PH7 \ttbar samples.

The inclusive \amc \ttbar sample uses the same scale settings and the same \pythiaa version as the PP8 \ttbar sample and is referred to as aMC+P8  \ttbar sample.

\end{description}



%The intrinsic uncertainty of the nominal PP8 \ttbb samples is expressed by the simultaneous variation of the renormalization and factorization scales ($\mu_R$ and $\mu_F$) by a factor two up and down. 
%The \texttt{RadiationUp} variation has the renormalization and factorization scales decreased by a factor of two, the \varc upward variation of the A14 parameter set and the \hdamp parameter doubled. The \texttt{RadiationDown} variation has the renormalization and factorization scales increased by a factor of two, the \varc downward variation and the nominal value of \hdamp.

%The scale uncertainties of the nominal PP8 \ttbar samples  are expressed by separate variations of the renormalization and factorization scales ($\mu_R$ and $\mu_F$) together with separate variations of \alphas in the initial and final-state radiation simulation of the parton shower. 
%as well as a separate variation of the \hdamp matching parameter.
%The relevant scales are independently varied by a factor two and one half.

%Both for ATLAS and CMS, uncertainties due to the PDF set are estimated as the envelope obtained from the replica provided by the NNPDF sets.

%The systematic uncertainty estimates due to scale variations are summarised in Table~\ref{tab:tttbbvariations}.

% old hdamp value in table \sum_{i=t,\bar{t},b,\bar{t}}m_{T}(i)$
\begin{sidewaystable}
  \centering
  \caption{\label{tab:ttbbsamples}
    Configurations used for the event generation of \ttbb processes and the predicted total cross section for events with at least one lepton. 
  }
  \vskip6pt
  {\scriptsize
    %\setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llllllllrrr}
      \toprule
      & name & ME & Generator & ME order & Shower & Tune\footnote{ ``default'' refers to the generator's default tune}%$^{\dagger}$ 
      & NNPDF PDF set & \hdamp & \bornzero & $\sigma^{\geq1 \text{lep}}$ [\si{\pico\barn}]  \\
      \midrule
      ATLAS  & PP8 \ttbb & \ttbb  & \powhegboxres & NLO & \pythia 8.210 & A14 & 4FS 3.0 NLO as 0118 & $H_T/2$ & 5 & 18.72 \\[3pt]
      \midrule
      ATLAS  & PP8 \ttbb $h_{\text{bzd}}$ 2  & \ttbb  & \powhegboxres & NLO & \pythia 8.210 & A14 & 4FS 3.0 NLO as 0118 & $\HT/2$ & 2 & 18.46  \\[3pt]
      
      ATLAS  & PP8 \ttbb dipole & \ttbb  & \powhegboxres & NLO & \pythia 8.210 & A14, dipoleRecoil\footnote{called by SpaceShower::dipoleRecoil "on"}& 4FS 3.0 NLO as 0118 & $\HT/2$ & 2 & 18.72 \\[3pt]
      ATLAS &PH7 \ttbb &  \ttbb &  \powhegboxres   & NLO & \herwig 7.13 & default & 4FS 3.0 NLO as 0118 & $\HT/2$ & 5 &18.47 \\[3pt]
      ATLAS & Sherpa \ttbb & \ttbb  & \sherpa 2.2.10 & NLO & \sherpa & default &  4FS 3.0 NNLO as 0118 & --- & --- & 20.24 \\ [3pt]
      \midrule
      % ATLAS & \ttbar & \sherpa 2.2.1 & \ttbar+0,1@NLO & \sherpa & default &  5FS 3.0 NNLO & --- & 451.78 \\
      % &        &               & +2,3,4@LO       & & & & & \\
      % ATLAS & \ttbb & \powheg v2    & NLO & \herwig 7.13 & default & 5FS 3.0 NLO  & \todo{?} & 451.78 \\[6pt] 
      % CMS   & \ttbb  & \amc 2.4.2    &  NLO    & \pythia 8.230 & CP5 & 4FS 3.1 NNLO as 0118 & --- & \ --- & todo{?} & \\ \midrule
      ATLAS & PP8  \ttbar & \ttbar  &\powheg v2    & NLO &\pythia 8.210 & A14 & 5FS 3.0 NLO  & $1.5 \cdot \mtop$ & 5 & 451.78\footnote{cross section predicted by NNLO calculation} \\[3pt]
      ATLAS &  PH7  \ttbar & \ttbar  & \powheg v2    & NLO &\herwig 7.13 & default & 5FS 3.0 NLO  & $1.5 \cdot \mtop$ & 5 & 451.78$^c$ \\[3pt]
      ATLAS &  aMC+P8  \ttbar & \ttbar & \amcnp      & NLO &  \pythia 8.210 & A14   &  5FS 3.0 NLO  & --- &  --- & 451.78$^c$\\[3pt] 
      
      \bottomrule\\[-2pt]
    \end{tabular}
  }
\end{sidewaystable}


\begin{sidewaystable}
  \centering
  \caption{\label{tab:ttbbscalechoices}
    Scale choices used in the event generation of \ttbb and \ttbar processes  for the different generators. %The scale settings of all \powhegboxres \ttbb samples, \powheg \ttbar, Sherpa and \amc \ttbar samples.
    %for the systematic variation samples  (ATLAS PP8 \bornzero2, PP8 dipole shower, PH7 \ttbb, PP8 \hdamp down)  reported in Table\,\ref{tab:ttbbsamples} correspond to the scale settings of the corresponding nominal sample. 
  }
  \vskip6pt
  \renewcommand{\arraystretch}{1.6}
  {\footnotesize
    \begin{tabular}{lcc}
      \toprule
      ME Generator 		& \muR & \muF \\
      \midrule
     
     ATLAS  \powhegboxres \ttbb & $\frac{1}{2} \sqrt[4]{m_\text{T,t}\cdot m_\text{T,\tbar}\cdot m_\text{T,b}\cdot m_\text{T,\bbar}}$
                                                         &  $\frac{1}{2} (m_{\text{T},\text{t}}+m_{\text{T},\overline{\text{t}}}+m_{\text{T},\text{b}}+m_{\text{T},\overline{\text{b}}}+m_{\text{T},\text{g}})$ \\
 %          \powhegboxres+\herwig 7   & {$\mu_\text{R} = \frac{1}{2} \sqrt[4]{m_\text{T,t}\cdot m_\text{T,\tbar}\cdot m_\text{T,b}\cdot m_\text{T,\bbar}}$} & --- \\
  %    & $\mu_\text{F} = \frac{1}{2} (m_{\text{T},\text{t}}+m_{\text{T},\overline{\text{t}}}+m_{\text{T},\text{b}}+m_{\text{T},\overline{\text{b}}}+m_{\text{T},\text{g}})$ & ---  \\ [10pt] 
            \sherpa 2.2.10                      &$ \frac{1}{2} \sqrt[4]{m_\text{T,t}\cdot m_\text{T,\tbar} \cdot m_\text{T,b}\cdot m_\text{T,\bbar}}$ 
                                         &$ \frac{1}{2} (m_{\text{T},\text{t}}+m_{\text{T},\overline{\text{t}}}+m_{\text{T},\text{b}}+m_{\text{T},\overline{\text{b}}}+m_{\text{T},\text{g}})$   \\
      \midrule
%            \powheg+\pythia 8 (5FS \ttbar)		& \multicolumn{2}{c}{$\mu_\text{R,F} = \sqrt{m_\text{t}^2 + p_\text{T, t}^2}$} \\
 %    \powheg+\herwig 7.13    & \multicolumn{2}{c}{$\mu_\text{R,F} = \sqrt{m_\text{t}^2 + p_\text{T, t}^2}$} \\[10pt]
         ATLAS \powheg \ttbar	& $ \sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}$ & $\sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}$\\
       
%      \powheg+\herwig 7.13    & \multicolumn{2}{c}{$\mu_\text{R,F} =\sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}$}  \\[10pt]

      
%      \sherpa 2.2.1 (5FS \ttbar)			& $\mu_\text{R,F} = \sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}$ & --- \\
   ATLAS aMC \ttbar  & $ \sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}$ & $ \sqrt{0.5 \cdot (m_\text{T,t}^2 + m_\text{T,\tbar}^2)}  $ \\
      \bottomrule
    \end{tabular}
  }
  \renewcommand{\arraystretch}{1.0}
\end{sidewaystable}



\begin{table}
  \caption{Systematic variations of scales in the matrix element and parton shower codes used for all comparisons presented here.}
  \label{tab:scalevariations}\label{tab:ttbbvariations}
  \vskip6pt
  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lcc}
    \toprule
    Variation &  \\
    \midrule
    Scale variation ME & \multicolumn{2}{c}{\muR $\times$  0.5 \muF $\times$ 0.5;  \muR $\times$ 2 \muF $\times$ 2} \\
   % ISR variation (PS) & \varc A14 tune$^{\dagger}$ & $\alpha_{s}^{\text{ISR}} \times 0.5, 2.0$ \\
    ISR variation (PS) &  \multicolumn{2}{c}{$\alpha_{\text{s}}^{\text{ISR}} \times 0.5, 2.0$} \\
    FSR variation (PS) & \multicolumn{2}{c}{$\alpha_{\text{s}}^{\text{FSR}} \times 0.5, 2.0$} \\
 %   $h_{\text{damp}}$ & --- & $h_{\text{damp}} \times 0.5, 2.0$ \\
    \bottomrule
   % \multicolumn{3}{l}{\footnotesize
    %$^{\dagger}$ $\alpha_{s}^{\text{ISR}}$ varied between 0.115--0.140    }
  \end{tabular}
  \renewcommand{\arraystretch}{1.0}
\end{table}

\newpage
\subsection{Object reconstruction and fiducial volume}\label{sec:rivet}
The object and event selection applied in this comparison study is defined at particle-level.
All objects are defined using stable final state particles with a mean lifetime of $\tau > 3\times 10^{-11}$~s. Jets are reconstructed from all stable final state particles (but excluding leptons and neutrinos from the top quark decay chain) using  the anti-$k_{\mathrm{t}}$ jet algorithm~\cite{Cacciari:2008gp,Cacciari:2011ma} with a radius parameter of $R = 0.4$. Jets which contain at least one ghost-associated~\cite{Cacciari:2008gn} $B$-hadron with transverse momentum (\pt) of $\pt\geq5$\,GeV are defined as \bjets, all other jets are considered "light" jets. The four-momentum of the bare leptons from top quark decay are modified ("dressed") by adding the four-momenta of all radiated photons within a cone of size $\Delta R=0.1$.  All objects are considered within pseudo-rapidity $|\eta| \leq 2.5$ and with $\pt>27$\,GeV for leptons and  $\pt>25$\,GeV for jets and \bjets .

Leptons are removed if they are separated from a jet by less than $\Delta R=0.4$, where $\Delta R = \sqrt{(\Delta \eta )^2 + (\Delta \phi)^2}$.
Events are selected with at least four \bjets, and further separated into two analysis regions: events with exactly one lepton and at least six jets (single lepton channel) and events with exactly two leptons and at least four jets (dilepton channel). %The object reconstruction and region definitions are summarised in Tables\,\

A set of observables  relevant for the \ttHbb analysis is studied within this fiducial phase space. All observables are studied for both the single lepton and the dilepton channel, however only the variables listed in Table\,\ref{tab:variables} are shown in the following figures, as no significant qualitative difference is observed between the different top quark decay channels.

%, , , , , , $N_{jets}$, 
\begin{table}[hb]
  \centering
  \caption{
    The list of observables used for the comparison of the generators for the \ttbb process.
    % The variable $\Delta R$ is calculated as $\Delta R = \sqrt{(\Delta \eta )^2 + (\Delta \phi)^2}$ .
  }\label{tab:variables}
  \vspace{0.25cm}
  {\small
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lll}
      \toprule
      Variable & Description  & Channel \\
      \midrule
      $\Delta R_{bb}^{\text{min} \Delta R}$ & $\Delta R$ of the two \bjets in the event which are closest in $\Delta R$ \,\,\,& dilepton \\ 
      $m_{bb}^{\text{min} \Delta R}$  & Invariant mass of the two \bjets closest in $\Delta R$                & dilepton \\ 
      $N_{\text{jets}}$   & Number of  jets in the event (all jet  flavours)      & dilepton    \\
      Light jet \pt  & Transverse momentum of the light jets in the event & dilepton \\
      \midrule
      $N_{\text{\bjets}}$   & Number of \bjets in the event      & single lepton  \\
      $\HT^{\text{jets}}$ & Scalar sum of \pt of jets in the event (all jet flavours) & single lepton \\
      % $N_{b-jets}$ & Number of $b$-jets \\
      Leading \bjet \pt \,\,\,& \pt of $b$-jet with largest \pt in the event & single lepton \\
      % Sub-leading $b$-jet $p_T$ & $p_{T}$ of $b$-jet with second largest $p_T$ in the event \\
      % Third $b$-jet $p_T$ & $p_{T}$ of $b$-jet with third largest $p_T$ in the event \\
      Fourth \bjet \pt & \pt of \bjet with fourth largest \pt in the event & single lepton\\
      % \HT & Scalar sum of all jet and lepton \pt in the event \\
      % \HT($b$-jets) & Scalar sum of all $b$-jet \pt in the event \\
      
      % All $b$-jet $p_T$ & $p_{T}$ of all $b$-jets in the event \\
      % Average $\Delta R (b,b)$ & Average over $\Delta R(b, b)$ build from all 2 $b$-jet combinations in the event \\ 
      
      % $\Delta R (b,b)$ (leading) & $\Delta R$ of the two leading $b$-jets in the event \\
      
      % $m (b,b)$ (leading) & Invariant mass of the two leading $b$-jets \\
      
      % $p_T (b,b)$ (leading) & Transverse momentum of the system with the two leading $b$-jets \\
      \bottomrule
    \end{tabular}
    \renewcommand{\arraystretch}{1.0}
  }
\end{table}




\subsection{Results}\label{sec:results}
Three sets of generator predictions are compared on the observables given in Table~\ref{tab:variables} as follows. All comparisons  are performed with respect to the  \ttbb PP8 sample.
 The PP8 \ttbb sample and the alternative predictions are normalised to an integral of 1, after all selections and in each histogram individually for a shape-only comparison.
The scale uncertainty variations on PP8 \ttbb are derived as  listed in  Table\,\ref{tab:scalevariations}  and the differences are added in quadrature to form the  shaded area displayed in the figures.
%...scale uncertainties are added and include normalisation differences with respect to the central value. 

Figure~\ref{fig:comp1} shows the nominal \ttbb predictions compared to the nominal predictions used in the early Run-2 analyses.  Significant differences between the PP8 \ttbb predictions and the PP8 \ttbar predictions  are observed in $\Delta R_{\bbbar}^{\text{min} \Delta R}$, the jet multiplicity and in the number of events with more than four \bjets. 

%For the RadiationUp uncertainty, an alternative sample with different \hdamp was used, here the number of events (not the sum of weights) was scaled to the central value.
%The central value of the PP8 \ttbar and the other three generators are normalised to 1. The first ratio plot shows the ratio of the different MC samples to PP8 \ttbar from the upper plot, where the colour scheme is given in the legend. The list of the validation variables for this comparison is presented in this note summarised in Table~\ref{tab:ttbb_varlist}.

In Figure~\ref{fig:comp2}, the nominal PP8 \ttbb prediction is compared to all generator variations potentially considered for modelling uncertainty for the ATLAS \ttHbb analysis, i.e.\ variations in \powhegboxres and \pythiaa parameter settings as well as \sherpa as alternative generator. As already discussed in~\cite{ttbbpubnote}, the parameter $\bornzero$ has only a minor influence on the observables. Interestingly, predictions of \powhegboxres matched to \pythiaa with dipole shower and  matched to \herwig parton shower  are similar and both show a significant decrease with respect to the nominal PP8 \ttbb  in the jet multiplicity and \HT. \sherpa differs up to  10--20\,\% in all distributions  mostly towards the edges of the phase space. Differences are in jet kinematics and in particular increasing differences towards high values are observed for $\Delta R_{\bbbar}^{\text{min} \Delta R}>1.5$.

%In the b-jet pair invariant mass variables $\mathrm{M_{bb}^{max P_T}}$ and $\mathrm{M_{bb}^{min \Delta R}}$ shown in Figures~\ref{ttbb:MbbmaxPT} and~\ref{ttbb:MbbminDR}, the largest difference is seen between the Sherpa \ttbar and all other samples.
%Two types of b-jet pairs are defined: one pair is build from the two b-jets with the highest \pt sum, called $\text{max}\pt$, and one pair from the two b-jets which are closest in $\Delta R$, called $\text{min}\Delta R$ . The invariant mass of the b-jet pairs are shown in Figures~\ref{ttbb:MbbmaxPT} and~\ref{ttbb:MbbminDR}, the largest difference is seen between the Sherpa \ttbar and all other samples.
%
%Differences are also observed in the \HT distributions, particularly in the 3b selection. In \HT of all b-jets, as in Figures~\ref{ttbb:HTbjets}, one observes a difference between PP8 \ttbar and the samples with b-jets in the matrix element, while in \HT of all light jets, shown in Figure~\ref{ttbb:HTljets}, a difference between the 4 and 5 flavour schemes can be seen. The jet multiplicity, as in Figure~\ref{ttbb:Njets}, has poor agreement among the generators for large jet multiplicities.
%Lastly, differences among the samples are shown for the $\eta_{\text{jet}}$ distribution, in Figure~\ref{ttbb:jeteta}.

%The second ratio plot shows the relative uncertainty of the radiation variations on PP8 \ttbar, shown as the ratio of the varied sample to the nominal for two cases described above, where the scale and A14 Eigentune parameters are either varied simultaneously (black) or individually and then summed following the CMS approach (red). \hdamp variations are only considered for the first case.
%In Figure~\ref{fig:comp3}, the CMS nominal PP8 \ttbb prediction is compared to generator variations considered for the CMS \ttHbb analysis. The scale uncertainties, which include the scale variations in the matrix element and the parton shower, are significantly larger than the differences observed for the different \hdamp variations, except at very low \HT and low leading \bjet \pt where the \hdamp down variations shows up to 20\,\% differences.
%Significant statistical fluctuations are observed at regions of low event yields, which are, however, not expected to be relevant for the analysis.

Finally, Figure~\ref{ttbb:comp4} shows the distributions used to estimate  the systematic modelling uncertainties of the first full Run-2 analysis by ATLAS~\cite{ttHbb}.  The uncertainty on the \ttbb PP8 prediction is estimated by assigning the relative difference between PP8 \ttbar and alternative \ttbar predictions listed in Table\,\ref{tab:ttbbsamples} to the \ttbb prediction. %Due to displaying purposes, the  PP8 \ttbar prediction is not shown. 

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/dR_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/m_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/N_Jets_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/all_lfjets_pt_geq4b_geq4j_dil.pdf}
  
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/N_b_Jets_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/ht_had_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/lead_bjet_pt_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_ATLAS_CMS_ME_PS/fourth_bjet_pt_geq4b_geq6j_ljets.pdf}
  \caption{
    Comparison of  PP8 predictions for \ttbb and \ttbar with the described settings using the observables defined in Table~\ref{tab:variables} in the fiducial analysis phase space.  %The central value of the PP8 \ttbb and PP8 \ttbar predictions are normalised to 1. 
    All predictions are normalised to 1. The error bands contain the scale variations (matrix element and parton shower) for  the PP8 \ttbb (blue) sample. Statistical uncertainties are indicated by vertical lines. 
    The ratio shows the different curves divided by the PP8 \ttbb prediction.
  }\label{fig:comp1}
\end{figure}



\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/dR_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/m_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/N_Jets_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/all_lfjets_pt_geq4b_geq4j_dil.pdf}
  
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/N_b_Jets_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/ht_had_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/lead_bjet_pt_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ATLAS_ME_PS_Var/fourth_bjet_pt_geq4b_geq6j_ljets.pdf}
  \caption{
    Comparison of PP8 predictions for \ttbb with different matching and parton shower settings and \sherpa. 
    All distributions  are normalised to 1. The ratio shows the different curves divided by PP8 \ttbb. The error band contains the scale variations (matrix element and parton shower) as defined in the text for the PP8 \ttbb sample. Statistical uncertainties are indicated by vertical lines.
  }\label{fig:comp2}
\end{figure}


  



\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/dR_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/m_bb_closest_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/N_Jets_geq4b_geq4j_dil.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/all_lfjets_pt_geq4b_geq4j_dil.pdf}
  
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/N_b_Jets_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/ht_had_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/lead_bjet_pt_geq4b_geq6j_ljets.pdf}
  \includegraphics[width=0.4\textwidth]{Plots/ttbb/Comp_April2022/PP8_ttbb_ttbar_Gen_ATLAS_CMS_ME_PS/fourth_bjet_pt_geq4b_geq6j_ljets.pdf}
  \caption{
    Comparison of  predictions used for the systematic uncertainties of the first full Run-2 analysis  by ATLAS~\cite{ttHbb}. 
    All distributions are normalised to 1. The ratio shows the different curves divided by PP8 \ttbb. The blue error band contains the scale variations (matrix element and parton shower) as defined in the text for the PP8 \ttbb sample. Statistical uncertainties are indicated by vertical lines.
  }\label{ttbb:comp4}
\end{figure}


\subsection{Conclusions}
 Comparisons of generator predictions used by ATLAS in a typical phase space of the \ttHbb measurement were presented. Two sets are used for comparison: the generators used in the most recent published analyses involving \ttbar inclusive predictions based on 5FS PDFs to estimate uncertainties and the set of generators in the future effort using \ttbb calculations at NLO based on 4FS PDFs. 
 
 %The PP8 predictions based on 5FS and 4FS PDFs only show minor shape differences in the \bjet \pt, however significant differences in the angular distance and the mass distribution of the \bbbar system and the jet multiplicity. The PP8 and \sherpa predictions based on \ttbb ME calculation agree well in most observables, only the \bjet \pt differs slightly, leading to up to 20\% differences also in \HT. These differences are of similar order as the variations of different parton showers  matched to \powhegboxres. It is interesting to note that  the angular difference between the closest \bjets in \sherpa differs at very high $\Delta R$ from all \powhegboxres based predictions. The variation of the \powhegboxres internal parameter \bornzero has  only a minor effect on the predictions. \\
 The difference between the predictions exceeds the uncertainties from the scale variations both for the uncertainties considered in the published \ttHbb analysis and  for the future analyses. 
  Smaller uncertainties due to the choice of  parton shower and NLO generator   are  observed when  estimating them based on     \ttbb ME  predictions  compared to the previously used \ttbar ME matched predictions. \\
 These distributions will be used in a future comparison of  theory  uncertainties between ATLAS and CMS. 
  %Despite differences in the set-up of the nominal \ttbb generators, only small differences are observed. The internal \powhegboxres parameters have only very limited effect on the predictions in the studied phase space.
